Reasoning about Ambiguous Definite Descriptions

Natural language reasoning plays an increasingly important role in improving language models' ability to solve complex language understanding tasks. An interesting use case for reasoning is the resolution of context-dependent ambiguity. But no resources exist to evaluate how well Large Language Models can use explicit reasoning to resolve ambiguity in language. We propose to use ambiguous definite descriptions for this purpose and create and publish the first benchmark dataset consisting of such phrases. Our method includes all information required to resolve the ambiguity in the prompt, which means a model does not require anything but reasoning to do well. We find this to be a challenging task for recent LLMs. Code and data available at: https://github.com/sfschouten/exploiting-ambiguity

==> glossary.tex <==
\newglossaryentry{linkprediction}
{
    name=Link Prediction,
    description={}
}

\newglossaryentry{kge}
{
    name=Knowledge Graph Embedding,
    plural=Knowledge Graph Embeddings,
    description={}
}



==> sections/X_neale_notes.tex <==
% Some notes from reading Stephen Neale's `Descriptions' 

\section{Neale Notes}

Definite, indefinite, demonstrative descriptions.
Possessive descriptions? (e.g. Our president)


Russel proposed a quantificational semantics of definite descriptions.
This has been challenged by many different philosophers.
One kind of challenge focuses on use of `the F' sentences which are used as shorthands for a particular entity, as if the description were a name.
Grice and Searle disagree, they say that what is \textit{said} is still a real definite description with Russelian semantics, but that people may still use such phrases pragmatically in order to convey something about a particular entity, which could be possible if interlocutors know of each other who is meant by a given definite description.


There are cases when people use definite descriptions in ways that seemingly do not comply with the quantificational account.
An example sentence is given ``John's murderer is insane.''. When this sentence is uttered by a detective standing over the dead body of John, having no idea yet who murdered him, then the use is certainly quantificational. But, when the sentence is uttered in a courtroom where John's murderer is currently standing trial, it seemingly is used as an ordinary referring expression.

Some have used this to argue for a semantic distinction between these two cases. 
Others (e.g. Grice) argue that this can be explained under a more general phenomenon, where there is a difference between the \textit{proposition expressed} and the \textit{proposition meant}.

Summary of four arguments for a semantic distinction:
\begin{itemize}
    \item Argument from misdescription: produce cases where Russelian and referring accounts differ in truth value, then appeal to intuition.
    \item Argument from incompleteness: examples such as `the table' are ``incomplete'' definite descriptions, thinking of them as referring expressions is supposed to fix this.
    \item Argument from opacity: examines descriptions in non-extensional contexts, where non-Russelian accounts are supposed to resolve or circumvent problems to do with scope, variable binding, and opacity.
    \item Argument from anaphora: 
\end{itemize}

We distinguish between the linguistic meaning of a an expression $\zeta$, and the semantical value of particular dated utterance \textit{u} of $\zeta$.
Expressions have meanings, utterances have values.

The semantical value of an utterance of a sentence is a proposition $\phi$.
The semantical value of an utterance of a subsentential expression $\alpha$ is whatever the utterance of $\alpha$ contributes to the identity of the proposition expressed by the utterance of the sentence $\phi$ of which $\alpha$ is a constituent.


`that man' vs. `the man I demonstrated' ...


Neale reaches the (according to him) Gricean view that we can distinguish three separate notions regarding the ``meaning'' of a sentence $\phi$ uttered by a speaker $S$ on a given occasion: 
\begin{enumerate}
    \item the linguistic meaning of the sentence $\phi$;
    \item the semantical value of the utterance relative to the context of utterance (proposition expressed); and 
    \item what S meant by uttering $\phi$ (the proposition meant).
\end{enumerate}



